Learning Sparse Rewarded Tasks from Sub-Optimal Demonstrations

Model-free deep reinforcement learning (RL) has demonstrated its superiority on many complex sequential decision-making problems. However, heavy dependence on dense rewards and high sample-complexity impedes the wide adoption of these methods in real-world scenarios. On the other hand, imitation learning (IL) learns effectively in sparse-rewarded tasks by leveraging the existing expert demonstrations. In practice, collecting a sufficient amount of expert demonstrations can be prohibitively expensive, and the quality of demonstrations typically limits the performance of the learning policy. In this work, we propose Self-Adaptive Imitation Learning (SAIL) that can achieve (near) optimal performance given only a limited number of sub-optimal demonstrations for highly challenging sparse reward tasks. SAIL bridges the advantages of IL and RL to reduce the sample complexity substantially, by effectively exploiting sup-optimal demonstrations and efficiently exploring the environment to surpass the demonstrated performance. Extensive empirical results show that not only does SAIL significantly improve the sample-efficiency but also leads to much better final performance across different continuous control tasks, comparing to the state-of-the-art.

==> sections/judy/introduction_backup.tex <==
%!TEX root = ../../main.tex

\section{Introduction}
Recent years witnessed the tremendous success of Reinforcement Learning (RL) in various tasks such as game playing \cite{mnih2015human,silver2017mastering} and robotics control \cite{gu2017deep}. However, these successes are typically restricted to domains with simulated environment, where millions of samples can be accessed at a negligible cost. In fact, the issue of high sample-complexity has largely prevented RL algorithms to scale to real-world settings. 
%
Towards resolving this challenge of sample-inefficiency, researcher have investigated approaches of exploiting prior knowledge to facilitate the RL process. Among those efforts, \textit{Imitation Learning (IL)} and \textit{Learning from Demonstrations (LfD)} are approaches that can effectively reduce the sample size by referencing to the expert demonstrations \cite{ho2016generative} or oracle policy \cite{sun2017deeply,gu2017deep,hester2018deep}. 


Reinforcement Learning (RL) solves sequential decision making problems by learning a policy to behave in a Markov decision Process via reward feedback.
% \judycom{Challenges}
There are two major challenges in RL: sample complexity and exploration.
% \judycom{Explain challenges}
Due to the delayed and noisy reward settings, it is highly expensive for RL policies to collect samples from the environment, especially for environments with high-dimensional observations or action spaces.
% 
Moreover, such high sample complexity prevents RL agents from efficient exploration. Most RL algorithms rely on random exploration approaches such as $\epsilon$-greedy~\cite{van2016deep} or adding noise actions~\cite{fujimoto2018addressing}, or use entropy-maximized learning objectives~\cite{haarnoja2018soft}, which implicitly encourage exploration.

While traditional RL struggles with these two challenges to improve policy, there are emerging approaches to achieve expert-level performance from limited expert demonstrations by Imitation Learning (IL)~\cite{ziebart2008maximum,ho2016generative,kostrikov2019imitation}. 
%
Compared with traditional RL, one merit of IL approaches is their effectiveness even when there is no reward feedback from the environment.
% 
One way to achieve IL is through the Inverse Reinforcement Learning (IRL), which aims at recovering a reward function that best explains the behavior of the expert demonstrations, and then performs RL on the learned reward distribution.
%
Recent advances in IL directly recover the expert policy by matching of stationary state-action distributions between the expert policy and the learned policy~\cite{ziebart2008maximum,ho2016generative,kostrikov2019imitation}, which avoids the cost in recovering the reward function. 

Among them, on-policy IL approaches such as Generative Adversarial Imitation Learning (GAIL) still require large number of samples from the environment. Recent success on off-line IL \cite{kostrikov2019imitation} can further boost the sample efficiency of the imitation process with minimal requirement of samples from the environment.
%such as Generative Adversarial Imitation Learning (GAIL) \cite{} and ValueDICE \cite{}, 
Despite their success, a major limitation of these IL approaches is that the asymptotic performance of their learned policies are bounded by the performance of given expert demonstrations, and further exploration is suppressed if the policy behavior deviates from the demonstrations. This becomes a major issue when the provided demonstrations are sub-optimal, despite the fact that sub-optimal demonstrations are typically much easier to be obtained than near-optimal ones. 

Another approach that leverages the behavior of experts is \textit{Learning from Demonstration} (LfD). Combined with value-based RL framework, LfD works by putting demonstration data in an replay buffer and treated them as self-generated samples to accelerate the sampling efficiency~\cite{vevcerik2017leveraging,hester2018deep}. 
%
Although the performance of the learned policy is not necessarily bounded by the quality of given demonstration, one drawback of LfD is that the demonstration data are not fully utilized as much as IL. Compared with IL, LfD needs more demonstration data to conduct efficient learning. Moreover, LfD approaches require dense reward feedbacks from environment for policy updates.


In this paper, we tackle the problem setting where an agent is provided with a \textit{limited} number of demonstrations from a \textit{sub-optimal} teacher; and the MDP feedback is extremely sparse such that only an episodic reward is provided once the agent reaches a terminal state.
%  
This is a very practical problem setting, as many real-world applications hardly have well crafted rewards for per-step action, but provide a general feedback whenever the task is done.
%
Besides, it is over-enthusiastic to assume the existence of expert behavior and also extremely costly to obtain near-optimal expert trajectories. In practice, we can be provided with limited demonstrations from a teacher to start with, whose performance is better than random decisions but may be still far away from experts.
%
%We address the problem of learning from limited, sub-optimal demonstrations. In this setting, we consider a MDP without dense rewards and only an episodic reward is provided once the task is terminated. We aim to efficiently recover the demonstration performance via off-policy learning, and gradually surpass the performance of the given demonstrations. Since the given demonstration is suboptimal and limited, the agent is allowed to sample from the environment for exploration.

To learn from this challenging problem setting, we propose a \textit{Self-Adaptive Imitation Learning (SAIL)}, an off-policy approach which leverages the low-quality demonstrated samples to quickly recover the teacher's performance by IL, and dynamically adjust the learning objective to surpass the demonstrated performance through RL, based on sparse guidance from episodic feedbacks. 
%
We highlight three components of our approach: (1) formulating the learning objective as exploration-based imitation learning, which encourages policy to imitate the teacher while pushing the policy away from previously learned ones; (2) selectively replacing the teacher demonstrations with self-explored trajectories to jump out of the restrictions of sub-optimal demonstrations; (3) further improving the sample efficiency by treating the given demonstrations as self-generated samples to boost initial learning performance; 

We conduct extensive empirical studies on physical locomotion tasks with high-dimensional state and action spaces, and compare the proposed SAIL with the state-of-the-art. Experimental results show that SAIL outperforms all baselines cross different tasks, with much higher sample efficiency and near-optimal asymptotic performance. 





==> sections/judy/method_backup.tex <==
\section{Background}
\subsection{Preliminaries} \label{sec:preliminaries}
We consider a standard Markov Decision Process defined as a tuple $ \cM=(\cS, \cA, \cT, r, \gamma, \mu_0, \cS_0)$, where $\cS$ and $\cA$ are the state and action space;
%
$\cT(s'|s,a)$ denotes the transition probability from state $s$ to $s'$ upon taking action $a$; 
%
$r(s, a)$ is the reward function;
%
$\gamma$ is a discounted factor;
%
$\mu_0$ is the initial state distribution with $s_0 \sim \mu_0$.
%
$\cS_0$ is the set of terminate states or \textit{absorbing states}. 
%
Any absorbing state will always transit to itself and yield zero rewards \cite{sutton2018reinforcement}. 
%  
We define the return for a trajectory $\tau=\{(s_t,a_t)\}_{t=0}^\infty$ as $R_t = \sum_{k=t}^{\infty} \gamma ^{k-t}r(s_t,a_t)$.
%
For episodic tasks with bounded sequence length, its return can be reduced as $R_t = \sum_{k=t}^{T} \gamma ^{k-t}r(s_t,a_t)$, where $T$ is the steps to reach the absorbing state.
%
The purpose of reinforcement learning is to learn a policy $\pi:~ \cS \to \cA $ to maximize the returns of trajectories visited by this policy.

Another important notation throughout this paper is the \textit{occupancy measure} of a policy $\pi$, defined as: 
%$\mu_\pi^t(s,a)=\cP(s_t=s,a_t=a|\cT,\pi)$, 
\begin{align} \label{eq:occupancy}
   \mu^\pi(s,a)=\sum_{t=0}^{\infty}\gamma^t \mu_\pi^t(s,a)
\end{align} 

The \textit{normalized discounted stationary distribution} of $\pi$ is therefore:
\begin{align*}
   d^\pi(s,a)= (1 - \gamma) \mu^\pi(s,a)
\end{align*} 

The objective of Equation \ref{eq:obj1} can be rewritten as maximizing the following:
\begin{align}
   \eta(\pi) &= \cE_{(s,a) \in \cS \times \cA}\big[\mu^\pi(s,a)r(s,a)\big] \nonumber \\
   &= \frac{1}{1 - \gamma}\cE_{(s,a) \sim d^\pi}\big[r(s,a)\big] 
\end{align}

% \begin{align} \label{eq:obj2}
%    \eta(\pi) = \cE_{\rho_{\pi}(s,a)} \big [   R(s,a) \big ] 
% \end{align}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Adversarial Imitation Learning}
Generative Adversarial Imitation Learning (GAIL) addresses the imitation learning task from the perspective of distribution matching. Given a set of expert demonstrations $\RE$ regarding an expert policy $\pi_E$ and its stationary state-action distribution is $\dE$, 
GAIL proposes to learn a policy $\pi$ to minimize the JS divergence between $d_\pi$ and $\dE$:
\begin{align*}
   &\arg\min_{\pi} D_{JS}(d_\pi, \dE) - \lambda H(\pi)
   %&\arg\min{\pi} \max_{D\in(0,1)^{\cS \times \cA}} \\
   %& \cE_{(s,a) \sim d_\pi}[\log(1 - D(s,a))] + \cE_{(s,a) \sim \dE}[\log( D(s,a))] - \lambda H(\pi)
\end{align*}

where $\lambda H(\pi)$ is an entropy term inspired by maximum entropy Inverse Reinforcement Learning (IRL) \cite{ziebart2008maximum,ziebart2010modeling}. 
GAIL shows that this objective can be gained by solving its dual as a min-max problem. Specifically, a discriminator $D$ is trained to learn the lower-bound of $D_{JS}[d_
\pi, \dE]$ and a policy $\pi$ is trained to improve this lower-bound, with the following objective:
\begin{align} \label{obj:gail}
   \min_\pi \max_{D} \cE_{d^\pi}[\log(1 - D(s,a))] + \cE_{\dE}[\log( D(s,a))] 
\end{align}
%where $\cE_{d^\pi}$ indicates that the state-actions are sampled from the stationary distribution of policy $\pi$.
For a fixed policy $\pi$, $D$ is trained to distinguish state-actions sampled from $\pi$ and the expert. It can be derived that the output of an optimized discriminator $D^*$ satisfies \cite{goodfellow2014generative}:
$ D^*(s,a) = \frac{\dE}{\dE + d_\pi} $.

Given a discriminator $D$, $\pi$ is trained in an on-policy fashion with a shaped reward function: $$r'(s,a) = -\log(1-D(s,a))$$
%
GAIL proves that optimizing the accumulated rewards of $r'(s,a)$ performs matching of occupancy measure between the policy and the expert. 
%
Since GAIL requires the occupancy measure of the learning policy $\pi$, most extended work of GAIL applies to on-policy algorithms. 
%
% Off-policy imitation learning approaches leverage a replay buffer $R$ to address sample inefficiency, and the objective of the learning policy $\pi$ becomes:

% \begin{align} \label{eq:obj3}
%    \min_{\pi} \max_{D} &\cE_{(s,a)\sim \dB}[\frac{d_{\pi}(s,a)}{d_{\dB}(s,a)}\log(1-D(s,a))] \nonumber \\
%    + &\cE_{s,a\sim \dE}[\log(D(s,a))]
% \end{align}

% $\frac{d_{\pi}(s,a)}{\dB(s,a)}$ is the importance weight to recover the gap between stationary distributions represented by replay buffer $\RB$ and a learned policy $\pi$. 

\subsection{Problem Setting}
We address the problem of learning from a environment with \textit{sparse, episodic} feedbacks: no rewards are given when a policy collects samples from the environment, except an episodic reward provided when the task is terminated. We denote samples from such environment as $\{s,a,s',i,r_e\}$, where $i$ is an indicator of whether a terminal(absorbing) state is reached:
\begin{equation}
   i(s,a,s') =
     \begin{cases}
       1 & \text{if $s' \in \cS_0$}\\
       0 & \text{otherwise} \nonumber
     \end{cases}       
 \end{equation}

 Note that we do not have access to the immediate reward of each transition $r(s,a)$. Instead, an episodic reward $r_e$ is provided whenever the policy reaches a terminal state:
\begin{equation}
   r_e(s_t,a_t, s_{t+1}) =
     \begin{cases}
       \sum_{i=0}^{t} r(s_t,a_t) &\text{if $s_{t+1} \in \cS_0$} \\
       0 & \text{otherwise} \nonumber
     \end{cases}       
 \end{equation}

In such problem setting, traditional RL approaches face challenges of high sample complexity. It may take long time for a policy to explore meaninglessly before reaching a terminal state.
%
To alleviate the learning difficulty, the policy is also provided with a few demonstrations from a \textit{sub-optimal} teacher. Pure imitation learning on the teacher may save the costs of random explorations. However, the asymptotic performance of the learning policy will be upper-bounded by the teacher's performance.
%
Since the given demonstrations are in low-quality, the policy is allowed to collect additional samples from the environment for exploration.

To sum-up, we start learning with an random policy $\pi_0$, a replay buffer with teacher demonstrations $\BE$, and a self replay buffer of transitions sampled from the random initial policy: $B=\{(s,a,s',i,r_e)\sim \pi_0\}$.
 
To quantify the teacher's demonstrations, we make the following necessary assumption: 
{\assumption{ \label{assumption:expert}
In early learning stages, following trajectories of the given demonstrations yields better rewards than following the policy $\pi$. Specifically, there exists $\delta \geq 0$, \st  
   $$\cE_{(s,a) \sim \dE}[r(s,a)] - \cE_{(s,a)\sim d_{B}}[r(s,a)] > \delta$$
}}
Our learning objective is to efficiently recover the teacher's policy based on its demonstrations, and gradually surpass the teacher to reach near-optimal performance via off-policy reinforcement learning. 
%
Although Assumption \ref{assumption:expert} is made only for early learning stages, we will show later that our designed method naturally makes this assumption tenable throughout the learning process.
%

\section{Methodology}
\subsection{Objective}  
We define our objective as exploration-based imitation learning: we train a policy $\pi$ which yields a stationary state-action distribution $d_\pi$ to optimize the following objective: 
{\objective \label{obj:primal}{
\begin{align} 
   &~~~~~~~~\max_\pi ~ J(\pi) \nonumber  \\ 
   = &- D_{\KL}[d_\pi || \dE] + D_{\KL}[d_\pi || d_{B}] \label{eq:obj-primal1}\\ 
   =  &~\cE_{(s,a) \sim d_\pi}[-\log \frac{d_\pi(s,a)}{\dE(s,a)}]  +  \log \frac{d_\pi(s,a)}{\dB(s,a)}] \nonumber\\
   =  &~\cE_{(s,a) \sim d_\pi}[\log \frac{\dE(s,a)}{\dB(s,a)}] \nonumber %\label{eq:obj-primal2}
\end{align} }}
 
While the first term in Equation \ref{eq:obj-primal1} encourages distribution match between $d_\pi$ and $\dE$, the second term of maximizing $D_\KL[d_\pi |\dB]$ is counter-intuitive at first sight. In our problem setting, maximizing $D_\KL[d_\pi |\dB]$ actually serves as an objective for exploration. Since $\dB$ can be treated as the state-action distribution of a mixture of previously learned policies, maximizing $\cE_{(s,a)\sim d_\pi}[\log\frac{d_\pi(s,a)}{\dB(s,a)}]$ encourages visiting state-actions that are rarely seen by previously learned policies: policy $\pi$ is encouraged to put more \textit{support} where $\dB < d_\pi$.
%
Encouraging the maximum of $D_\KL[d_\pi || d_B]$ alone leads to unbounded exploration.
%
However, combined with the first term in Equation \ref{eq:obj-primal1}, this exploration is guided in the direction of decreasing $D_\KL[d_\pi || \dE]$.



\subsection{Benefits of exploration-driven objective given sub-optimal demonstrations:}
An alternative objective which appears more to intuition would be: 
\begin{align}  
   \max_\pi &  - D_\KL[d_\pi || \dE] + \lambda H(\pi) \nonumber\\%\tilde{J}_{\dE}(\pi) =
   =  \max_\pi &\cE_{(s,a) \sim d_\pi}[\log \frac{\dE(s,a)}{d_\pi(s,a)}] + \lambda H(\pi) \nonumber
\end{align}
where $H(\pi)$ being a entropy term controlled by $\lambda \geq 0$.
%

We interpret the benefits of maximizing $E_{d_\pi}[\log(\frac{\dE}{\dB})]$ instead of $E_{d_\pi}[\log(\frac{\dE}{d_\pi})]$ from two perspectives. 
%
On one hand, it accelerates the imitation learning process by forcing policy $\pi$ to selectively build support. 
%
Maximizing $\cE_{(s,a) \sim d_\pi}[\log \frac{\dE(s,a)}{\dB(s,a)}]$ can be considered as a process of policy selection: for state-actions where the expert has visted more frequently than the past learned policies, $\pi$ is encouraged to build support on those state-actions: $d_\pi(s,a) > 0$ where $\dE(s,a) > \dB(s,a)$. 
%
Intuitively, it means we trust the expert more than the previously learned policies, which is a fair policy selection given assumption \ref{assumption:expert}.
%
We will show later in this paper with experiments that the objective of $\max_\pi E_{d_\pi}[\log(\frac{\dE}{\dB})]$ encourages more efficient-exploration compared with $\max_\pi E_{d_\pi}[\log(\frac{\dE}{d_\pi})]$.

On the other hand, it encourages exploration.
%
An optimal solution to $\max_\pi \cE_{d_\pi}[\log \frac{\dE(s,a)}{d_\pi(s,a)}]$  is a policy that exactly recovers the teacher's occupancy with $d_\pi^*= \dE$.
%
In our problem setting, however, the teacher demonstrations are sub-optimal, and a policy that exactly matches the teacher's occupancy does not necessarily lead to good performance.
%
Moreover, maximizing $E_{d_\pi}[\log(\frac{\dE}{d_\pi})]$ restricts $\pi$ from further exploring occupancies that deviates from $\dE$.
%  


\subsection{Self Adaptive Imitation Learning}  
Based on the above problem-setting and objective, we design Self Adaptive Imitation Learning(SAIL), an algorithm that enables exploration-driven imitation learning.
%
SAIL maintains two replay-buffers $\RE$ and $\RB$, for caching teacher demonstrations and samples collected by the learning policy, respectively. We alternatively train three components: a discriminator $D$ that serves as the reward shaper, a critic $Q$ to minimize the Bellman error using the shaped rewards, and a actor $\pi$ to maximize the accumulated shaped rewards. Note that $D$, $Q$, and $\pi$ are all learned off-policy. 
%
Its pseudo-code is shown in Algorithm \ref{alg:version2}. We highlight three aspects of our algorithm that make SAIL effective:

(1) \textbf{Estimating the ratio of $\log(\frac{\dE}{\dB})$ by learning a discriminator $D$ in an off-policy fashion}: $D$ is trained to differentiate samples from $\RB$ and samples from $\RE$ by maximizing the following equation:
$$\max_{D} J_D = \cE_{\dB}[\log(1 - D(s,a))] + \cE_{\dE}[\log( D(s,a))] $$
%
Given fixed $\dE$ and $\dB$, if we train the discriminator to optimality, its output for any state-action pair will obtain:
$D^*(s,a)=\frac{\dE(s,a)}{\dE(s,a) + \dB(s,a)}$ \cite{goodfellow2014generative}. %Therefore, $-\log(1-D^*(s,a)) = \log (1+ \frac{\dE(s,a)}{\dB(s,a)}) $

Prior work such as GAIL trains the discriminator with on-policy samples to estimate $\frac{\dE}{d_\pi}$ instead of $\frac{\dE}{\dB}$. We will show later in this paper that, compared with its on-policy counterpart, this off-policy discriminator aligns with our proposed objective and encourages exploration more efficiently, in the case of sub-optimal teacher demonstrations.
 


(2) \textbf{Automatically replacing teacher demonstration $\dE$ with self-generated trajectories}: 
%
whenever the policy $\pi$ collects a trajectory with higher episodic scores than a threshold $C_\dE$, we add them to the teacher's demonstration buffer. 
%
Powered by an exploration-based objective, policy $\pi$ can gradually replace sub-optimal demonstrations with self-generated demonstrations that are better than the teacher. 
%
During the learning process, the threshold $C_\dE$ is simultaneously updated as the lowest episodic score in the demonstration buffer $\RE$: $$C_\dE = \min_{r^j_e \neq 0}\{r^j_e |(s_j,a_j, \dots, r^j_e \in \RE) \}$$
%
Unlike other approaches which learn a critic based on environment rewards, we leverage the sparse rewards only from environment for selecting better demonstrations, and performs imitation learning on those demonstrations without the need to access true immediate reward for each transition step.
%

%Assumption \ref{assumption:expert} renders a reasonable objective: we want to imitate the expertise by maximizing -$D_\KL[d_\pi ||\dE ]$, whereas stays away from novice by maximizing ($D_\KL[d_\pi || \dB]$), as long as the expertise is indeed better than the novice.
%To keep it this constraint tenable, we manipulate two replay buffers by selectively adding new samples of interactions to them. 
% Especially, for any trajectory $\tau^i$ collected by policy, $\pi$ $\tau^i = \{s^i_0, a^i_0, s^i_1, \dots, s^i_{T_i} \}$ with episodic reward $r_e^i$, we add it into $\dE$ whenever $r_e^i$ reaches the score lower-bound of trajectories stored in $\dE^+$, otherwise add it to $\dB$:
% \begin{align*}
%    \dE \leftarrow \dE &\cup \tau^i \text{~if} C_\dE = \min \{{r_e^j ~|\tau^j \in C_\dE \}} \\
%    \dB \leftarrow \dB &\cup \tau^i \text{~otherwise} 
% \end{align*} 
 

(3) \textbf{Fully leveraging teacher demonstrations to boost imitation learning}:
Besides imitation learning on the teacher's demonstrations, we also use them to update $Q$ as well as $\pi$ in early learning stages, as if they were generated by the learning policy itself.
% 
The ratio of samples from teachers demonstrations are dynamically adjusted, and will drop to 0 once the learning policy is able to generate trajectories better than the teacher.
%
We will theoretically draw a connection between learning from demonstrations and a regularized imitation learning objective in Section \ref{sec:lfd-theory}, and also show that this approach further warmups the imitation learning process by ablation study.

Specifically, this process can be formulated as training a Q network parameterized by $\phi$ to minimize the expectation of Bellman error over a mixture of two replay buffers:
\begin{align}
   \arg\min_\phi J(Q_\phi) := \alpha ~&\cE_{(s,a, s) \sim \dE}[\frac{1}{2}(Q_\phi(s,a)-y)^2] \nonumber \\
   + (1-\alpha)&\cE_{(s,a, s') \sim \dB}[\frac{1}{2}(Q_\phi(s,a)-y)^2] \label{sobj:q}
\end{align}
where $y = r'(s,a) + \gamma \bar{Q}(s',\pi_\theta(s'))$; $\bar{Q}$ is a target Q network to stabilize training; $r'(s,a)=-\log(1-D(s,a))$ is the shaped reward using discriminator's output; $\alpha \geq 0$ is the regularization coefficient.

Following the idea of DDPG \cite{lillicrap2015continuous}, we train a deterministic policy $\pi$ parameterized by $\theta$ by performing off-policy gradient to maximize $Q$:
\begin{align*}
   %\triangledown_{\theta} J(\pi_\theta) = &\cE_{(s,a)\sim \dB}[\triangledown_\theta Q(s, a|a=\pi_\theta(a))|] \\
   (1-\alpha) \cE_{\dB}[\triangledown_a Q(s, a)|\triangledown_\theta \pi(s)] ~+  
   \alpha \cE_{\dE}[\triangledown_a Q(s, a)|\triangledown_\theta \pi(s)]
   %\max_\pi J_\pi:= \cE_{(s,a)\dMIX}[Q(s,a)]
\end{align*} 

where $\alpha$ is the same coefficient as in Equation \ref{sobj:q}. In practice, We initialize $\alpha=0.5$ and dynamically reduce it to zero.
  

\iffalse
\section{Regularized Off Policy Optimization}
Given expert replay buffer $\RE$, a convex function $f$, we can define the primal objective as:

\begin{align*} 
   \max_\pi J_{\RE, f}(\pi) = \cE_{s,a\sim \pi}[r(s,a)] - \alpha D_f(d_\pi || \dE)
\end{align*}

$D_f(d_\pi || \dE)$ is the $f-$divergence between stationary distribution derived from policy $\pi$ and stationary distribution from the expert replay buffer $\RE$.

Its dual objective function is:
\begin{align*}
   \max_\pi &\min_{x: \cS \times \cA \to \RR} \hat{J}_{\RE, f}(\pi, x) = \\
   &\cE_{(s,a) \sim d_\pi}[r(s,a) - \alpha.x(s,a)] + \alpha \cE_{(s,a)\sim \dE}[f_*(x(s,a))]
\end{align*}

Define $v: \cS \times \cA \to \RR$ as:
\begin{align*}
   v(s,a) &= r(s,a) - \alpha x(s,a) + \cE_{s' \sim \cT, a' \sim \pi}[v(s',a')] \\
   &= -\alpha x(s,a)  + \cB_\pi v(s,a)
\end{align*}

Replacing $x(s,a)$ with $(\cB_\pi v - v)(s,a)/\alpha$ yields:
\begin{align} \label{eq:opod}
   &\max_\pi \min_{x: \cS \times \cA \to \RR} \hat{J}_{\RE, f}(\pi, x) \nonumber \\
   &=\cE_{(s,a) \sim d_\pi}[r(s,a) - \alpha.x(s,a)] + \alpha \cE_{(s,a)\sim \dE}[f_*(x(s,a)] \nonumber \\
   &\max_\pi \min_{v: \cS \times \cA \to \RR} \hat{J}_{\RE, f}(\pi, v) \nonumber \\
   &=(1-\gamma)\cE_{(s_0 \sim \mu_0,a_0 \sim \pi(s_0))}[v(s_0,a_0)] + \nonumber \\ 
   &~~~~~~~~~~~~~~~~~~\alpha \cE_{(s,a)\sim \dE}[f_*((\cB_\pi v - v)(s,a)/\alpha)]  
\end{align}

Provided that $f(x)=(x-1)^2$ and $f_*(x)=\frac{1}{4}x^2+x$, Equation \ref{eq:opod} is equivalent to:
\begin{align*}
   &\max_\pi \min_{v: \cS \times \cA \to \RR} \hat{J}_{\RE, f}(\pi, v) \nonumber \\ 
   =&(1-\gamma)\cE_{(s_0 \sim , a_0)}[v(s_0,a_0)] + \cE_{(s,a)\sim \dE}[\frac{1}{4\alpha}\delta(s,a)^2 + \delta(s,a)]  
\end{align*}
where $\delta(s,a) = \alpha x(s,a) = (\cB_\pi v - v) (s,a)$
\fi 


%\subsection{Off Policy Gradient Distribution }
% Since the KL-divergence between two distributions $P$ and $Q$ is defined as:
% \begin{align*}
%    \KL(P || Q ) = - \cE_{x \in \cX}[P(x)\log Q(x)] - \cH(Q(x))
% \end{align*}
% We can rewrite Equation \ref{obj:AIRL} in terms of $\KL(d_\pi || \dE)$ and $\KL(d_\pi || \dB)$:
% \begin{align*}
%    &\max_\pi \cE_{(s,a) \sim d_\pi(s,a)} \big[\log(\dE(s,a)) - \log(d_R(s,a)) \big]  \\
%    = &\max_\pi\Big[-\KL(d_\pi || \dE) -\cH(d_\pi) + \KL(d_\pi || \dB) + \cH(d_\pi)\Big]  \\
%    = &\min_\pi\Big[\KL(d_\pi || \dE) - \KL(d_\pi || \dB)  \Big]  
% \end{align*}

% So we can see there is a tradeoff between keeping a large replay buffer $\cR$ and obtaining a minimal distribution discrepancy between $d_\pi$ and $\dE$.

\subsection{Connections from Off-Policy Learning to Density Regularization} \label{sec:lfd-theory}
Objective \ref{obj:primal} assumes that we have access to \textit{online} samples from the environment to get expectations over $d_\pi$. 
% 
In practice, we learn $Q$ and $\pi$ based on samples from a mixture of replay buffers, which brings a concern that the learned policy diverges from optimizing the original objective.
% 
In this section, we provide a perspective which interprets an off-policy gradient approach as performing density regularization in addition to the on-policy objective.
%
We will show that this reformulation can also explain the benefits of learning from teacher demonstrations.
%as it enhance the density match between the learning policy and the teacher.

Considering a regularized version of Objective \ref{obj:primal}: 
{\objective \label{obj:primal2}
\begin{align} %\label{obj:primal2} 
   \max_\pi & \tilde{J}_{f, \beta, \lambda}(\pi) \nonumber \\ 
   =&{J}(\pi)   - \lambda D_f[d_\pi || \dbeta ] \nonumber
   %=&\cE_{(s,a) \sim d_\pi}[\log \frac{\dE(s,a)}{\dB(s,a)}] - \lambda D_f[d_\pi || \dbeta]  \nonumber
\end{align}}
This objective is our original max-return objective, regularized by the divergence between $d_\pi$ and a stationary distribution $\dbeta$.
%
Specifically, $D_f[P||Q]$ denotes a $f$-divergence between distributions $P$ and $Q$, with f being a convex, non-negative function \cite{nowozin2016f}: 
$$D_f[P||Q] = \int_\cX q(x) f\big(\frac{p(x)}{q(x)}\big)$$

$\dbeta$ can be arbitrary stationary state-action distributions.
%
Let us set $\dbeta$ as the stationary distribution of the off-policy data that we use to learn the policy. Especially, in our case: $$\dbeta = \dMIX = (1-\alpha) \dB + \alpha \dE$$ with $\alpha \geq 0$. 
%
Then we can re-write the regularized objective as following:
\begin{align*}
   %\max_\pi & \tilde{J}_{\dE, \dB, f, \lambda}(\pi)=
   \max_\pi \cE_{(s,a) \sim d_\pi}[\log \frac{\dE(s,a)}{\dB(s,a)}] - \lambda D_f[d_\pi || \dMIX]  
\end{align*}
 
Solving the above objective can be considered as solving a dual problem by transforming the $f$-divergence to its variational form \cite{nguyen2010estimating}:
\begin{align} 
   \max_\pi & \tilde{J}_{f,\beta,\lambda}(\pi) = \max_\pi \min_{x: \cS \times \cA \to \RR} \tilde{J}_{f,\beta,\lambda}(\pi, x) \nonumber \\
= ~&\cE_{ d_\pi}[ \log \frac{\dE(s,a)}{\dB(s,a)} - \lambda.x(s,a)] + \lambda \cE_{\dMIX}[f_*(x(s,a))] \nonumber
\end{align}
Where $f_*(x)$ is the convex conjugate function of $f$ \cite{nachum2020reinforcement}.
%
Inspired by DualDICE \cite{nachum2019dualdice}, let use define $Q: \cS \times \cA \to \RR$ as a fixed point of certain Bellman operation:
\begin{align*}
   Q(s,a) &= -\lambda x(s,a)  + \cB_\pi Q(s,a)  
\end{align*}

where $\cB_\pi Q(s,a) = r'(s,a) +  \cE_{s' \sim \cT(s,a), a' \sim \pi}[Q(s',a')]$ and $r'(s,a) = \log \frac{\dE(s,a)}{\dB(s,a)}$. 

%$\cE_{d_\pi}[r'(s,a) - \lambda.x(s,a)] = \cE_{(s_0 \sim \mu_0,a_0 \sim \pi(s_0))}[Q(s_0,a_0)] $

By changing variables with $x(s,a)= \frac{1}{\lambda}(\cB_\pi Q - Q)(s,a)$ as well as a series of reduction of telescoping \cite{nachum2019dualdice,nachum2019algaedice}, we can again re-write the dual objective as following:
\begin{align} \label{eq:dual}
   &\max_\pi \min_{x: \cS \times \cA \to \RR} \tilde{J}_{f,\beta,\lambda}(\pi, x)  \nonumber\\
  % =&\cE_{d_\pi}[r'(s,a) - \lambda.x(s,a)] + \lambda \cE_{\dMIX}[f_*(x(s,a)] \nonumber \\
   = &\max_\pi \min_{Q: \cS \times \cA \to \RR} \tilde{J}_{f,\beta,\lambda}(\pi, Q) \nonumber \\
   =&(1-\gamma)\cE_{(s_0 \sim \mu_0,a_0 \sim \pi(s_0))}[Q(s_0,a_0)] ~+ \nonumber \\ 
   &~~~~~~~~~~~~~~~~~~\lambda \cE_{(s,a)\sim \dMIX}[f_*(\frac{1}{\lambda}(\cB_\pi Q - Q)(s,a))]  
\end{align}
%Reduction from $\cE_{d_\pi}[r'(s,a) - \lambda.x(s,a)]$ to $\cE_{(s_0,a_0 )}[Q(s_0,a_0)]$ leverages the telescoping proposed in DualDICE \cite{nachum2019dualdice}.

Up to now, a rising question is How does this objective connected with our current learning approach? It turns out that by a proper choice of $f(x)=f_*(x)=\frac{1}{2}x^2$, the above Equation becomes resemblant of an off-policy actor-critic objective:
$$\max_\pi \min_Q (1-\gamma)\cE_{(s_0 ,a_0)}[Q(s_0,a_0)] + \frac{1}{2\lambda} \cE_{\dMIX}[((\cB_\pi Q - Q)(s,a))^2] $$

%In practice, when performing actor-critic training, target $\pi$ and target $Q$ networks are widely adopted to stabilize training \cite{lillicrap2015continuous,fujimoto2018addressing}.

\judycom{(TBD: gap between this objective and our proposed objective .)}

By iteratively learning $\pi$ and $Q$ using off-policy data sampled from distribution $\dMIX$, we can treat this learning process as a way of regularizing the divergence between $d_\pi$ and $\dMIX$.
%
When $\dMIX=\alpha \dE + (1-\alpha) \dB$ with a positive $\alpha$, it expediates the density match between $d_\pi$ and $\dE$.
%
We will show by ablation study in Section \ref{sec:abstudy} that, learning from teacher demonstrations, i.e setting a positive $\alpha$, indeed speed up the imitation learning performance in early training stages.



\iffalse
\section{Theoretical foundations} \label{sec:lfd-theory}
Although balancing the exploration and imitation seems appealing,
one limitation for the proposed objective function in \eq{\ref{eq:obj-primal1}} is that we assume the access to \textit{on-policy} samples from the environment to get expectations over $d_\pi$. This on-policy requirement would
largely limit the sample-efficiency of our approach. 
% 
% In practice, we learn $Q$ and $\pi$ based on samples from a mixture of replay buffers, which brings a concern that the learned policy diverges from optimizing the original objective.
% 
In this section, we provide a concrete theoretical foundation that
builds upon previous arts~\cite{nachum2019algaedice} to transfer
the on-policy objective into a practical off-policy approach.
% perspective which interprets an off-policy gradient approach as performing density regularization in addition to the on-policy objective.
%
Furthermore, this reformulation also explain the benefits of learning from teacher demonstrations.
%as it enhance the density match between the learning policy and the teacher.

Considering a regularized objective: 
\begin{align} \label{obj:primal2}
   \max_\pi & \tilde{J}_{f, \beta, \lambda}(\pi) := {J}(\pi)   - \lambda D_f[d_\pi || \dbeta ] 
   %=&\cE_{(s,a) \sim d_\pi}[\log \frac{\dE(s,a)}{\dB(s,a)}] - \lambda D_f[d_\pi || \dbeta]  \nonumber
\end{align}
This objective is our original max-return objective in Equation \ref{eq:obj-primal2}, regularized by the divergence between $d_\pi$ and a stationary distribution $\dbeta$.
%
Specifically, $D_f[P||Q]$ denotes a $f$-divergence between distributions $P$ and $Q$, with f being a convex, non-negative function \cite{nowozin2016f}: 
$$D_f[P||Q] = \int_\cX q(x) f\big(\frac{p(x)}{q(x)}\big)$$

$\dbeta$ can be arbitrary stationary state-action distributions.
%
Let us set $\dbeta$ as the stationary distribution of the off-policy data that we use to learn the policy. Especially, in our case: $$\dbeta = \dMIX = (1-\alpha) \dB + \alpha \dE$$ with $\alpha \geq 0$. 
%
Then we can re-write the regularized objective as following:
\begin{align*}
   %\max_\pi & \tilde{J}_{\dE, \dB, f, \lambda}(\pi)=
   \max_\pi & \tilde{J}_{f, \beta, \lambda}(\pi) := \cE_{(s,a) \sim d_\pi}[\log \frac{\dE(s,a)}{\dB(s,a)}] - \lambda D_f[d_\pi || \dMIX]  
\end{align*}
 
Solving the above objective can be considered as solving a dual problem by transforming the $f$-divergence to its variational form \cite{nguyen2010estimating}:
\begin{align} 
   &\max_\pi \tilde{J}_{f,\beta,\lambda}(\pi) = \max_\pi \min_{x: \cS \times \cA \to \RR} \tilde{J}_{f,\beta,\lambda}(\pi, x) \nonumber \\
 &:=\cE_{ d_\pi}[ \log \frac{\dE(s,a)}{\dB(s,a)} - \lambda.x(s,a)] + \lambda \cE_{\dMIX}[f_*(x(s,a))] \nonumber
\end{align}
Where $f_*(x)$ is the convex conjugate function of $f$ \cite{nachum2020reinforcement}.
%
Inspired by DualDICE \cite{nachum2019dualdice}, let use define $Q: \cS \times \cA \to \RR$ as a fixed point of certain Bellman operation:
\begin{align*}
   Q(s,a) &= -\lambda x(s,a)  + \cB_\pi Q(s,a)  
\end{align*}

where $\cB_\pi Q(s,a) = r'(s,a) +  \cE_{s' \sim \cT(s,a), a' \sim \pi}[Q(s',a')]$ and $r'(s,a) = \log \frac{\dE(s,a)}{\dB(s,a)}$. 

%$\cE_{d_\pi}[r'(s,a) - \lambda.x(s,a)] = \cE_{(s_0 \sim \mu_0,a_0 \sim \pi(s_0))}[Q(s_0,a_0)] $

By changing variables with $x(s,a)= \frac{1}{\lambda}(\cB_\pi Q - Q)(s,a)$ as well as a series of reduction of telescoping \cite{nachum2019dualdice,nachum2019algaedice}, we can again re-write the dual objective as following:
\begin{align} \label{eq:dual}
   &\max_\pi \min_{x: \cS \times \cA \to \RR} \tilde{J}_{f,\beta,\lambda}(\pi, x)  = \max_\pi \min_{Q: \cS \times \cA \to \RR} \tilde{J}_{f,\beta,\lambda}(\pi, Q) \nonumber \\
   &:= (1-\gamma)\cE_{(s_0 \sim \mu_0,a_0 \sim \pi(s_0))}[Q(s_0,a_0)] ~+ \nonumber \\ 
   &~~~~~~~~~~~~~~~\lambda \cE_{(s,a)\sim \dMIX}[f_*(\frac{1}{\lambda}(\cB_\pi Q - Q)(s,a))]  
\end{align}
%Reduction from $\cE_{d_\pi}[r'(s,a) - \lambda.x(s,a)]$ to $\cE_{(s_0,a_0 )}[Q(s_0,a_0)]$ leverages the telescoping proposed in DualDICE \cite{nachum2019dualdice}.

Up to now, a rising question is How does this objective connected with our current learning approach? It turns out that by a proper choice of $f(x)=f_*(x)=\frac{1}{2}x^2$, the above Equation becomes resemblant of an off-policy actor-critic objective:
\begin{align}
   &~~~~~~~~~~~~\max_\pi \min_Q \tilde{J}_{f,\beta,\lambda}(\pi, Q)  := \nonumber \\
&(1-\gamma)\cE_{(s_0 ,a_0)}[Q(s_0,a_0)] + \frac{1}{2\lambda} \cE_{\dMIX}[((\cB_\pi Q - Q)(s,a))^2] 
\end{align}

%In practice, when performing actor-critic training, target $\pi$ and target $Q$ networks are widely adopted to stabilize training \cite{lillicrap2015continuous,fujimoto2018addressing}.

\judycom{(TBD: gap between this objective and our proposed objective .)}

By iteratively learning $\pi$ and $Q$ using off-policy data sampled from distribution $\dMIX$, we can treat this learning process as a way of regularizing the divergence between $d_\pi$ and $\dMIX$.
%
When $\dMIX=\alpha \dE + (1-\alpha) \dB$ with a positive $\alpha$, it expedites the density match between $d_\pi$ and $\dE$.
%
We will show by ablation study in Section \ref{sec:abstudy} that, learning from teacher demonstrations, i.e setting a positive $\alpha$, indeed speed up the imitation learning performance in early training stages.
\fi 


 

\iffalse
\subsection{Replay Buffer Regularization}
We collect transitions of our training policy into a replay buffer $\cR$, and alter the objective as:
\begin{align*}
   &\max_\pi \min_{v: \cS \times \cA \to \RR} \hat{J}_{\RE, f}(\pi, v) \nonumber \\ 
   =(1-\gamma)(1-\beta)&\cE_{(s_0 \sim \mu_0,a_0 \sim \pi(s_0))}[v(s_0,a_0)] ~~+ \nonumber \\
\beta &\cE_{(s,a)\sim \dB}[r(s,a) - (\cB_\pi v - v)(s,a)] ~~+ \\
   \alpha(1 - \beta) &\cE_{(s,a)\sim \dE}[f_*((\cB_\pi v - v)(s,a)/\alpha)] + \\
   \alpha \beta &\cE_{(s,a)\sim \dB}[f_*((\cB_\pi v - v)(s,a)/\alpha)] 
\end{align*}
\fi

%Based on this reward setting, the learning objective is same as: $r^(s,a)=\log \frac{D(s,a)}{1-D(s,a)}$
\iffalse
\judycom{\subsection{Objective derived from Soft Actor Critic}}

\begin{align} \label{obj:primal3} 
   &\max_\pi  J_{\dE, \dB, f}(\pi) \nonumber \\
   &= - D_{\KL}[d_\pi || \dE] + D_{\KL}[d_\pi || d_{B}]- \alpha H(\pi) \nonumber \\
   &=\cE_{(s,a) \sim d_\pi}[\log \frac{\dE(s,a)}{\dB(s,a)}] - \alpha H(\pi) \nonumber \\
   &=\frac{1}{1-\gamma}\cE_{(s,a) \sim \mu_\pi}[\log \frac{\dE(s,a)}{\dB(s,a)}] - \alpha H(\pi) \nonumber \\
   &=\frac{1}{1-\gamma}\sum_{t=0}^{T}\cE_{(s_t,a_t)\sim \mu_\pi^t}[\log\frac{\dE(s,a)}{\dB(s,a)} - \frac{\alpha}{1-\gamma} H(\pi(.|s))  ]
   %\mu_\pi^t(s,a)=\cP(s_t=s,a_t=a|\cT,\pi)
\end{align}
where $\mu_\pi$ is the occupancy measure of policy $\pi$, as defined in Section \ref{sec:preliminaries}.
\fi 
 
\iffalse
We collect transitions of our training policy into a replay buffer $\dB$, and train a discriminator to differentiate samples from expert buffer $\dE$ and self replay buffer $\dE$ by maximizing the following objective:
\begin{align} \label{eq:discriminator}
   \max_{D} &\dE_{(s,a)\sim d_\dB}[ \log(1-D(s,a))] \nonumber \\
   + &\dE_{s,a\sim \dE}[\log(D(s,a))]
\end{align}

Given fixed $\dE$ and $\dB$, if we train the discriminator to optimality its output for any state-action pair will obtain:
$D^*(s,a)=\frac{\dE(s,a)}{\dE(s,a) + \dB(s,a)}$ \cite{goodfellow2014generative}. 

Given a discriminator $D$, we shape the imitation reward as $r'(s,a) = \log(D(s,a))-\log(1-D(s,a))$ for any state-action pairs.

A policy $\pi$ is learned to optimize the expectation of accumulated rewards:
\begin{align*}
\pi^* = \argmax_\pi &\cE \big[ \sum_{t=0}^{\infty} \gamma^t r'(s,a) | 
s_0 \sim \mu_0, \\
&\forall t, a_t \sim \pi(s_t), s_{t+1} \sim \cT(s_t,a_t)\sim \pi \big]
\end{align*} 

Assuming that the discriminator is trained to be optimal, the shaped reward function regarding an optimal discriminator would be $r^*$:
\begin{align*}
   r^* &= \log(D^*(s,a)) - \log(1-D^*(s,a)) \\
       &= \log(\dE(s,a)) - \log(\dB(s,a))
\end{align*}
Based on this reward setting, learning an optimal policy is equivalent to optimizing the following objective:

\begin{align} \label{obj:AIRL}
   \max_\pi &\cE \big[ \sum_{t=0}^{\infty} \gamma^t r^*(s,a) | 
s_0 \sim \mu_0, \nonumber \\
&\forall t, a_t \sim \pi(s_t), s_{t+1} \sim \cT(s_t,a_t)\sim \pi \big] \nonumber \\
=  \max_\pi &\cE_{(s,a) \sim d_\pi(s,a)} \big[ r^*(s,a)\big] \nonumber \\
=  \max_\pi &\cE_{(s,a) \sim d_\pi(s,a)} \big[\log(\dE(s,a)) - \log(d_R(s,a)) \big]  
\end{align}
\fi


\iffalse

\subsection{Distribution Divergence Regularization by learning from Demonstrations}

Suppose we have access to a stationary state-action distribution $d_\beta$, then there is a one to one mapping between a policy $\pi_\beta(a|s)$ and $d_\beta$, $\st$ $\pi_\beta(a|s)= \frac{d_\beta(s,a)}{\sum_{a'\in \cA} d_\beta(s,a')} $, and the stationary state-action distribution generated by $\pi_\beta$ is $(1-\gamma)d_\beta$ \cite{syed2008game}. 

In the case of imitation learning, we are given a set of expert demonstrations $\RE$ from which an estimate of stationary state-action distribution $\dE$ can be derived. 
%  
The purpose of IL is to recover an expert policy $\pE$ whose normalized occupancy measure is $\dE$, even when the provided demonstrations are collected from a mixture of  policies or human supervisors.

We take training observations in $\RE$ as sampled from an expert policy $\pE$. When training on these dataset, we can rewrite the gradient of our policy as:
\begin{align*}
   \triangledown_\theta J(\theta) = \triangledown_\theta &\cE_{s\sim \rhoE}\big[ \sum_{a\in \cA} Q^\pi(s,a) \pi_\theta(a|s) \big] \\
   & \approx \cE_{s\sim \rhoE}\big[ \sum_{a\in \cA} Q^\pi(s,a) \pi_\theta(a|s) \big] 
\end{align*} 

where $\rhoE = \sum_{a\in \cA} \dE(s,a) \pi(a|s) $



The Q function for an ideal $\pE$ satisfies the Bellman Equation:
$$ \QE(s,a) \triangleq r(s,a) + \cB^\pE \QE(s,a)$$
where $\cB^\pi Q(s,a)$ is the Bellman operation: $$\cB^\pi Q(s,a)= E_{s'\sim \cT(s,a), a' \sim \pi}[Q(s',a')]$$

% For deterministic policy, we can rewrite it as:
% $$\cB^\pi Q(s,a)= E_{s'\sim \cT(s,a)}[Q(s',\pi(s'))]$$


In other words, its Q function minimizes the Bellman Equation over trajectories visited by the expert policy:

\begin{align*}
   \QE = \arg \min_{Q}  E_{(s,a) \sim \dE}\Big[\big(r(s,a) + \cB^\pE Q(s,a) - Q(s,a) \big)^2 ]
\end{align*}
% From the perspective of distribution matching, we aim to learn a policy $\pi$ to minimize the divergence between a normalized distribution $d_\pi$ and $\dE$:

% \begin{align*}
%    J(d_\pi, )
% \end{align*}



% define D_\pi
We care about three stationary distributions: $\dE$, $\dB$, $d_\pi$, which are the state-action distributions regarding the expert replay buffer $\RE$, self-generated replay buffer $\RB$, and the normalized stationary distributions generated by the target policy $\pi$.
%
We only have estimates of $\dE$ and $\dB$ but not $d_\pi$. 
%
\fi

\iffalse
\begin{align*}  
   \max_{\pi} \min_{D} &\cE_{s,a\sim \cR}[- \log(1- D(s,a))] \\
   + &\cE_{s,a\sim \RE}[-\log(D(s,a))]
\end{align*}

In an actor-critic off-policy RL framework, we learn a policy by learning a Q-function $Q_{\phi}$ to minimize the Bellman error, and use the learned $Q$ to update our policy:

$$Q \leftarrow \arg \min_Q || r(s,a) + \gamma \max_{a'}(Q(s',a')) - \bar{Q}(s,a)||^2$$
where $\bar{Q}$ is the target Q network. 

From the perspective of Q function, optimizing Q can be considered equivalent as minimizing the following objective:

\begin{align} \label{eq:Qobj}
   %&\max_{\pi} \cE_{s,a\sim \BMIX }[r(s,a)] \equiv \nonumber \\
   &\min_{Q} \cE_{s,a\sim R} \big || R(s,a) - Q(s,a) \big ||^2  \nonumber \\  
   &+  \cE_{s,a\sim R_E} \big || R(s,a) - Q(s,a) \big ||^2 
\end{align}
with $R(s,a)$ being the reward to go of state action $(s,a)$.
% 


For continuous action space with a deterministic policy, action with highest Q value is approximated as $\max_a Q(s,a) \approx Q(s,\pi_\theta(s))$. 
%
The policy $\pi_\theta$ is updated to ascend its gradient by chain-rule:
\begin{align*}
 \frac{d\pi}{d\theta}(s) \frac{dQ_\theta}{d_a}(s,a)
\end{align*}
\fi 
\iffalse
Since $Q(s,a)=\mu_\pi(s,a) r(s,a)$, 
and $\cE_{s,a\sim \RE} [R(s,a)]= \cE_{s,a\sim \RE} [Q^E(s,a)]$, where $Q^E(s,a) = \mu_E(s,a) r(s,a)$,
% 
the second part of Equation \ref{eq:Qobj} is therefore equivalent to:
\begin{align*}
   &\cE_{s,a\sim R_E} \big || R(s,a) - Q(s,a) \big ||^2 \\
   =&\cE_{s,a\sim R_E} \big || \hat{\mu}_E(s,a) r(s,a)-  \mu_\pi r(s,a) \big ||^2 \\
   =&\cE_{s,a\sim R_E} \big || \hat{\mu}_E(s,a) -  \mu_\pi  \big ||^2 r(s,a)^2
\end{align*}

So we can see that sampling from expert buffer to update the Q function as well as the policy serves as a regularization to minimize the divergence between $\mu_E$ and $\mu_\pi$.
\fi 

\iffalse
\subsection{Training Objective}
We use the TD3 framework to update our policy with a shaped reward function:
\begin{align} \label{obj:SAIL}
   \max_\pi &\cE \big[ \sum_{t=0}^{\infty} \gamma^t r(s,a) | 
s_0 \sim \mu_0, \nonumber \\
&\forall t, a_t \sim \pi(s_t), s_{t+1} \sim \cT(s_t,a_t)\sim \pi \big] \nonumber \\
=  \max_\pi &\cE_{(s,a) \sim d_\pi(s,a)} \big[ r(s,a)\big] \nonumber \\
\end{align}

where $r(s,a)=-\log(1-D(s,a))$.
\fi 

\iffalse
\subsection{Stabilize Learning by Support Set Matching}
To alleviate the error accumulation caused by out-of-distribution actions, we use Maximum Mean Discrepancy (MMD) to constrain the support-set matching between the training dataset distribution and the target policy.

Especially, given two distributions $P$ and $Q$ over a set $\cX$, and a feature map $\varphi: \cX \to \cH$, where $\cH$ is a Reproducing Kernel Hilbert Space (RKHS) on $\cX$, then the MMD between $P$ and $Q$ is:
\begin{align}
   \vMMD(P, Q) = || \cE_{x\sim P}[\varphi(x)] - \cE_{y\sim Q}[\varphi(y)] ||_{\cH} \nonumber
\end{align}
A sampled version of MMD using Gaussian kernel can be represented as:
\begin{align*}  
   &\vMMD(\{x_i \sim P \}^n_{i=1}, \{ y_j \sim Q \}_{j=1}^m) = \\
   &\frac{1}{n^2}\sum_{i,i'}k(x_i, x_{i'}) - \frac{2}{mn} \sum_{i,j}k(x_i, y_j) + \frac{1}{m^2}\sum_{j,j'}k(y_j,y_{j'}) 
\end{align*}


Combined with imitation learning and support set matching, the ultimate training objective of the target policy becomes:
% \begin{align} \label{obj:final} 
%    \max_\pi &\cE \big[ \sum_{t=0}^{\infty} \gamma^t r(s,a) | 
% s_0 \sim \beta, \forall t, a_t \sim \pi(s_t), s_{t+1} \sim \cT(s_t,a_t)\sim \pi \big] \nonumber \\ 
%    \text{s.t.} &\cE_{s \sim \BMIX }  [MMD \big(\pi(s), \BMIX(s) \big)] \leq \epsilon \nonumber
% \end{align} 
   
Where $\BMIX = \cR_{E} \cup \cR $ and $r(s,a) = - \log(1- D(s,a))$.
\fi
 
\begin{algorithm*}[tb]
   \caption{Self-Adaptive Imitation Learning}
   \label{alg:version2}
\begin{algorithmic}
   \STATE {\bfseries Input:} teacher replay buffer $\RE$ with demonstrations, 
   \STATE ~~~~~~~~~~~~self-replay-buffer $\RB$ with random transitions, temporary cache buffer $\cR_c$.  
   \STATE{~~~~~~~~~~~~absorbing states $S_0$, initial policy $\pi_\theta$, discriminator $D_w$, critic $Q_\phi$, batch size $N > 0$, coefficient $\alpha > 0$}
   %$\RE$ with trajectories $\{ \tau^E_1, \tau^E_2, \dots, \tau^E_N \big \}$
   %expert episodic scores $S_E= \big \{ e^E_1, e^E_2, \dots, e^E_N \big \}$.\STATE{Initialize policy $\pi_0$, discriminator parameters $w$, , expert-replay-buffer $\RE = \emptyset$,  maximum iteration $I$, warmup buffer size $B_W$, trajectory cache buffer $\cR_c$}
   %%% 
   % \FOR{$n=1$ {\bfseries to} $N$}
   % %\STATE sample expert transition $(s^E,a^E,., s^E)  \sim \dE$,   
   % \STATE $\RE \leftarrow \RE \cup \tau^E_i$.  
   % \STATE $\RE$.\code{scores} $\leftarrow \RE$.\code{scores} $\cup~ \{e^E_i \}$  
   % ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~$\star$ prepare expert-replay buffer
   % \ENDFOR
   %%% 
   % \FOR{$n=1$ {\bfseries to} $B_W$}
   % \STATE{ sample $(s,a,., s') \sim \pi_\theta$.}
   % %\STATE {$r' \leftarrow - \log \big (1-D_w(s, a) \big )$ }
   % \STATE { $\cR \leftarrow \cR \cup (s,a,., s')$.} ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~$\star$ prepare self-replay buffer
   % \ENDFOR 
   %%%%%%%%%
   \FOR{$n=1$, $\dots$} 
   \STATE {sample $(s,a,.,s', r_e) \sim \pi_\theta$, $\RB \leftarrow \RB \cup (s,a,.,s')$ , ~~~~~~~~~~~~~~~~~~~~~~~~~$\star$ store trajectories in self-replay buffer}
   \STATE {$\cR_c \leftarrow \cR_c \cup (s,a,., s')$
   ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~$\star$ cache current episode }
   \IF{$s' \in S_0$ }
      \IF {$r_e> \min_{r^j_e \neq 0} \{(r^j_e ~|~ (s_j, a_j, ., r^j_e) \in \RE\} $ ) }
      \STATE $\RE \leftarrow \RE \cup \cR_c$ 
      % 
      ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~$\star$ store good trajectories in expert-replay buffer  
      \STATE{$\alpha \leftarrow 0$}
      \ENDIF
      \STATE{$\cR_c \leftarrow \emptyset$
      %
      ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~$\star$ refresh cache buffer
      } 
   \ENDIF
   \STATE
   %%%%%%%%%
   \IF{ $n \mod \code{discriminator-update}= 0$} 
   \STATE  $\big \{ (s_i, a_i, ., ., .) \big \}_{i=1}^{N} \sim \RB, \big \{ (s^E_i, a^E_i, ., ., .) \big \}_{i=1}^{N} \sim \RE$   
   \STATE update $D_w$ by ascending gradient : ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~$\star$ optimize discriminator
   \STATE ~~~~~~~~~~~~~~~$\triangledown_w \frac{1}{N} \sum_{i=1}^{N}\big[ \log D \Big( s^E_i, a^E_i\Big) +  \log \Big( 1- D \big( s_i, a_i \big) \Big) \big]$ 
   %
   \ENDIF
   %%%%%%%%%
   \STATE
   \IF{ $n \mod \code{Q-update}= 0$}    
   \STATE{$\big \{ (s_i, a_i, ., s'_i, .) \big \}_{i=1}^{N} \sim \RB, \big \{ (s^E_i, a^E_i, ., s'^{E}_i, .) \big \}_{i=1}^{N} \sim \RE$ }
   \STATE{set $y_i= -\log(1-D(s_i,a_i)) + \gamma \bar{Q}(s'_i, \pi(s'_i))$ }
   \STATE{~~~~~$y^E_i= -\log(1-D(s^E_i,a^E_i)) + \gamma \bar{Q}(s'^E_i, \pi(s'^E_i))$ }
   \STATE update $Q_\phi$ by minimizing critic loss: ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~$\star$ optimize critic
   \STATE ~~~~~~~~~~~~~~~$J(Q_\phi) = \frac{1- \alpha}{N} \sum_i[(Q_\phi(s_i,a_i)-y_i)^2] +  \frac{\alpha}{N} \sum_i[(Q_\phi(s_i^E,a_i^E)-y^E_i)^2] $
   \ENDIF
   \STATE   
   \IF{ $n \mod \code{policy-update}= 0$}    
   %\STATE{$\big \{ (s_i, a_i, ., s'_i, .) \big \}_{i=1}^{B} \sim \RB, \big \{ (s^E_i, a^E_i, ., s'^{E}_i, .) \big \}_{i=1}^{B} \sim \RE$ }
   %\STATE $\tau_E =\big \{ (s^E_i, a^E_i, ., s'^{E}_i, .) \big \}_{i=1}^{B} \sim \RE$, $r'^E_i \leftarrow  - \log \big (1-D_w(s^E_i, a^E_i) \big )$ 
   %\STATE  $\tau = \big \{ (s_i, a_i, ., s'_i, .)\sim \RB \big \}_{i=1}^{N}  \cup \big \{ (s^E_i, a^E_i, ., s'^{E}_i, .)  \sim \RE \big \}_{i=1}^{N}$
   %\STATE $\tau$ = $\big \{ (s_i, a_i, ., s'_i, .) \big \}_{i=1}^{B} \sim \RB$, $\tau_E =\big \{ (s^E_i, a^E_i, ., s'^{E}_i, .) \big \}_{i=1}^{B} \sim \RE$
   %%%%%%%%% 
   \STATE{$\big \{ (s_i, a_i, ., s'_i, .) \big \}_{i=1}^{N} \sim \RB, \big \{ (s^E_i, a^E_i, ., s'^{E}_i, .) \big \}_{i=1}^{N} \sim \RE$ }

   \STATE update $\pi$ by sampled policy gradient:  ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~$\star$ optimize policy 
   %\STATE ~~~~~~~~~~~~~~~$J(\pi_\theta) \approx \frac{1}{2B} [(Q_\phi(s_i,a_i)-y_i)^2] + \frac{1}{B} [(Q_\phi(s_i^E,a_i^E)-y^E_i)^2] $
   \STATE ~~~~~~~~~~~~~~~$J(\pi_\theta) \approx \frac{1-\alpha}{N} \sum_{i}[\triangledown_a Q(s_i, a_i)|\triangledown_\theta \pi(s)] + \frac{\alpha}{N} \sum_{i}[\triangledown_a Q(s_i^E, a_i^E)|\triangledown_\theta \pi(s)]$
   %
   \ENDIF 
   \ENDFOR 
\end{algorithmic}
\end{algorithm*} 
 

  

==> sections/judy/sup_alg.tex <==
% !TEX ROOT=../../main.tex



 
 

==> sections/judy/sup_exp.tex <==
% !TEX ROOT=../../main.tex
\section{Implementation Details}
We implemented \SAIL based on open-sourced code from stable-baselines\footnote{https://stable-baselines.readthedocs.io/en/master/}.
%
We tested \SAIL on 4 physical locomotion tasks simulated by OpenAI MuJoCo\footnote{https://github.com/openai/mujoco-py}: \textit{Walker2d-v2, Hopper-v2, HalfCheetah-v2}, and \textit{Swimmer-v2}.
%
For each task, we generate teacher demonstrations by training a TD3 benchmark to sub-optimal performance, and store trajectories with triplets $(s_t, a_t, s_{t+1},.)$ in to the teacher replay buffer. 
%
The original locomotion tasks are all in dense-reward setting. To simulate a sparse feedback environment, we omit the immediate reward such that only an episodic reward is given when a complete trajectory is reached.

\SAIL is compared with 4 baselines that are mostly applicable to our problem setting: Behavior Cloning (BC), GAIL \cite{ho2016generative}, DAC \cite{kostrikov2018discriminator}, and POfD \cite{kang2018policy}.
% 
For \SAIL and DAC, $Q$ networks are trained by 1000 gradient steps every time after 1000 transitions are sampled from the experiments. 
%
Except for BC which does not need shaped rewards, all benchmarks adopt the same discriminator network architecture with 2 MLP layers, each of 256 hidden units. To alleviate the over-fitting issue for the discriminator, we adopt the gradient penalty loss as proposed for Wasserstein GANs \cite{gulrajani2017improved}, with a gradient penalty coefficient set as 10. 
%
Details about hyper-parameters are illustrated in Table 1 and Table 2.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[] 
    \begin{center}
    \begin{tabular}{lcc}   
        \toprule
    \textbf{Environment} & \multicolumn{1}{l}{\textbf{Self Buffer Size}} & \multicolumn{1}{l}{\textbf{Teacher Buffer Size}} \\
    \midrule
    HalfCheetah-v2       & $10^6$                                        & $10^4$                                           \\
    Swimmer-v2           & $10^5$                                        & $10^4$                                           \\
    Hopper-v2            & $10^6$                                        & $10^5$                                           \\
    Walker2d-v2          & $10^6$                                        & $10^4$    \\ 
    \bottomrule
    \end{tabular}
    \caption{Replay buffer Setting.}
    %\vskip 0.1in 
    %%%%%%
    \begin{tabular}{lccccc} 
        \toprule
    \textbf{Network} & \multicolumn{1}{l}{\textbf{Layer}} & \multicolumn{1}{l}{\textbf{Hidden Size}} & \multicolumn{1}{l}{\textbf{Gradient Penalty}} & \multicolumn{1}{l}{\textbf{Update Frequency /Env Steps}} & \multicolumn{1}{l}{\textbf{Gradient Steps}} \\
    \midrule
    Critic ($Q$)           & 2 MLP                                      & $400 \times 300$                         & N/A                                           & 1000                                                     & 1000                                        \\
    Actor ($\pi$)            & 2 MLP                                      & $400 \times 300$                         & N/A                                           & 2000                                                     & 1000                                        \\
    Discriminator ($D$)    & 2 MLP                                      & $256 \times 256$                         & 10                                            & 500                                                      & 10            \\                             
    \bottomrule
\end{tabular} 
\caption{Network hyper-parameter setting.}
\end{center} 
\end{table}
 

\section{Experimental Results in Evaluation Mode}
Besides the learning performance provided in the main paper, we also illustrate the performance of \SAIL and other baselines in \textit{evaluation} mode. As shown in Figure \ref{fig:ep1-sail-dynamic}, we evaluate each policy with 1 and 4 demonstration trajectories, respectively. This evaluation is performed whenever 2048 \textit{learning} steps have been taken. Different from \textit{learning} mode where action noises are added for exploration, during the evaluation mode, only deterministic actions are taken. Evaluation results verify that \SAIL performs consistently the best in both training and testing modes, with or without random action explorations.


\begin{figure*}[ht]
    \begin{center}  
        \hskip -0.1in
        \begin{minipage}[b]{.27\textwidth}
            \centerline{\includegraphics[width=\columnwidth]{figs/Walker2d-v2-ep1-dynamic-pofd-test.pdf}} 
            %\caption{Walker2d-v2}\label{ep4-walker}
        \end{minipage} %\hskip -0.3in %\qquad  
        \hskip -0.2in
        \begin{minipage}[b]{.27\textwidth}
            \centerline{\includegraphics[width=\columnwidth]{figs/Swimmer-v2-ep1-dynamic-pofd-test.pdf}}
            %\caption{Swimmer-v2}\label{ep4-swimmer}
        \end{minipage} \hskip -0.2in
        \begin{minipage}[b]{.27\textwidth}
            \centerline{\includegraphics[width=\columnwidth]{figs/Halfcheetah-v2-ep1-dynamic-pofd-test.pdf}}
            %\caption{Swimmer-v2}\label{ep4-swimmer}
        \end{minipage} \hskip -0.2in
        \begin{minipage}[b]{.27\textwidth}
            \centerline{\includegraphics[width=\columnwidth]{figs/Hopper-v2-ep1-dynamic-pofd-test.pdf}} 
        \end{minipage}%\qquad   

        \hskip -0.1in
        \begin{minipage}[b]{.27\textwidth}
            \centerline{\includegraphics[width=\columnwidth]{figs/Walker2d-v2-ep4-dynamic-pofd-test.pdf}} 
            %\caption{Walker2d-v2}\label{ep4-walker}
        \end{minipage} %\hskip -0.3in %\qquad  
        \hskip -0.2in
        \begin{minipage}[b]{.27\textwidth}
            \centerline{\includegraphics[width=\columnwidth]{figs/Swimmer-v2-ep4-dynamic-pofd-test.pdf}}
            %\caption{Swimmer-v2}\label{ep4-swimmer}
        \end{minipage} \hskip -0.2in
        \begin{minipage}[b]{.27\textwidth}
            \centerline{\includegraphics[width=\columnwidth]{figs/Halfcheetah-v2-ep4-dynamic-pofd-test.pdf}}
            %\caption{Swimmer-v2}\label{ep4-swimmer}
        \end{minipage} \hskip -0.2in
        \begin{minipage}[b]{.27\textwidth}
            \centerline{\includegraphics[width=\columnwidth]{figs/Hopper-v2-ep4-dynamic-pofd-test.pdf}} 
        \end{minipage}%\qquad   
    \caption{\textbf{Evaluation} curves of \SAIL and other baselines using 1 demonstration trajectory (upper panel) and 4 demonstration trajectories (lower panel) with sparse (episodic) rewards. Each unit in $x$-axis correspond to 2048 * 10 \textit{learning} steps, whereas $y$-axis shows the averaged \textit{evaluated} episode returns. We evaluate the policy by taking only deterministic actions sampled from the policy.}
    \label{fig:ep1-sail-dynamic}
    \end{center}
    \vskip -0.2in
\end{figure*}

\section{Algorithm}
The complete pseudo code for \SAIL is shown in Algorithm \ref{alg:version2}.

{\small{
\begin{algorithm*}[tb]
    \caption{Self-Adaptive Imitation Learning}
    \label{alg:version2}
 \begin{algorithmic}
    \STATE {\bfseries Input:} teacher replay buffer $\RE$ with demonstrations, 
    \STATE ~~~~~~~~~~~~self-replay-buffer $\RB$ with random transitions.  
    \STATE{~~~~~~~~~~~~initial policy $\pi_\theta$, discriminator $D_w$, critic $Q_\phi$, batch size $N > 0$, coefficient $\alpha > 0$} 
    %%%%%%%%%
    \FOR{$n=1$, $\dots$} 
    \STATE {sample trajectory $\tau \sim \pi_\theta$, $\RB \leftarrow \RB \cup \tau$ , ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~$\star$ store trajectories in self-replay buffer} 
     
       \IF {$r_e(\tau)> \min_{\tau'} \{(r_e(\tau') ~|~ \tau' \in \RE \} $ ) }
       \STATE $\RE \leftarrow \RE \cup \tau$ 
       % 
       ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~$\star$ store good trajectories in expert-replay buffer  
       \STATE{$\alpha \leftarrow 0$~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~$\star$ stop sampling from mixture of buffers}
       \ENDIF
       
     
    %\STATE
    %%%%%%%%%
    \IF{ $n \mod \code{discriminator-update}= 0$} 
    \STATE  $\big \{ (s_i, a_i, ., ., .) \big \}_{i=1}^{N} \sim \RB, \big \{ (s^{T}_i, a^{T}_i, ., ., .) \big \}_{i=1}^{N} \sim \RE$   
    \STATE update $D_w$ by ascending gradient : ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~$\star$ optimize discriminator
    \STATE ~~~~~~~~~~~~~~~$\triangledown_w \frac{1}{N} \sum_{i=1}^{N}\big[ \log D \Big( s^{T}_i, a^{T}_i\Big) +  \log \Big( 1- D \big( s_i, a_i \big) \Big) \big]$ 
    %
    \ENDIF
    %%%%%%%%%
    %\STATE
    \IF{ $n \mod \code{Q-update}= 0$}    
    \STATE{$\big \{ (s_i, a_i, ., s'_i, .) \big \}_{i=1}^{N} \sim \RB, \big \{ (s^{T}_i, a^{T}_i, ., s^{'{T}}_i, .) \big \}_{i=1}^{N} \sim \RE$ }
    \STATE{set $y_i= -\log(1-D(s_i,a_i)) + \gamma \bar{Q}(s'_i, \pi(s'_i))$ }
    \STATE{~~~~~$y^{'{T}}_i= -\log(1-D(s^{T}_i,a^{T}_i)) + \gamma \bar{Q}(s^{'{T}}_i, \pi(s^{'{T}}_i))$ }
    \STATE update $Q_\phi$ by minimizing critic loss: ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~$\star$ optimize critic
    \STATE ~~~~~~~~~~~~~~~$J(Q_\phi) = \frac{1- \alpha}{N} \sum_i[(Q_\phi(s_i,a_i)-y_i)^2] +  \frac{\alpha}{N} \sum_i[(Q_\phi(s_i^{T},a_i^{T})-y^{'{T}}_i)^2] $
    \ENDIF
    %\STATE   
    \IF{ $n \mod \code{policy-update}= 0$}    
    \STATE{$\big \{ (s_i, ., ., ., .) \big \}_{i=1}^{N} \sim \RB, \big \{ (s^{T}_i, ., ., ., .) \big \}_{i=1}^{N} \sim \RE$ }
    %\STATE{$\big \{ (s_i, a_i, ., s'_i, .) \big \}_{i=1}^{N} \sim \RB, \big \{ (s^E_i, a^E_i, ., s'^{E}_i, .) \big \}_{i=1}^{N} \sim \RE$ }
 
    \STATE update $\pi$ by sampled policy gradient:  ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~$\star$ optimize policy 
    %\STATE ~~~~~~~~~~~~~~~$J(\pi_\theta) \approx \frac{1}{2B} [(Q_\phi(s_i,a_i)-y_i)^2] + \frac{1}{B} [(Q_\phi(s_i^E,a_i^E)-y^E_i)^2] $
    \STATE $\triangledown_\theta J(\pi_\theta) \approx \frac{1-\alpha}{N} \sum_{i}[
       %
    %\triangledown_a Q(s_i, a_i)|\triangledown_\theta \pi(s)
    \triangledown_\theta \pi_\theta(s_i) \triangledown_a Q(s_i,a_i)|_{a_i=\pi_\theta(s_i)}
    %
    ] + \frac{\alpha}{N} \sum_{i}[
       %
       %\triangledown_a Q(s_i^E, a_i^E)|\triangledown_\theta \pi(s)
       \triangledown_\theta \pi_\theta(s_i^{T}) \triangledown_a Q(s_i^{T},a_i^{T})|_{a_i^{T}=\pi_\theta(s_i^{T})}
       %
       ]$
    %
    \ENDIF 
    \ENDFOR 
 \end{algorithmic}
 \end{algorithm*}   
 }}

==> sections/judy/sup_related_work.tex <==
% !TEX ROOT=../../main.tex

\section{Challenges faced by TD Learning on Sparse Rewarded Tasks}  
Temporal Difference (TD) Learning has been embedded in various value-based RL algorithms. Different from a Monte-Carlo approach which updates its estimation of $Q$-values based on completely sampled returns, TD learning leverages bootstrapping to update the $Q$-value $Q(s,a)$ with an immediate reward $r(s,a)$ and an estimated successor $Q(s', a')$: 
$$ Q(s,a) = r(s,a) + \gamma \cE_{s'\sim \cT, a \sim \pi(s')}[Q(s',a')]$$

TD-learning methods have achieved significant performance in tasks such as game playing or robotics control.
% 
Successes on these applications usually hinge on well-designed, dense reward feedbacks that are available at negligible costs in simulation but are difficult to access in real world scenarios.
%
For highly sparse-rewarded tasks, such as in our problem setting, the immediate rewards $r(s,a)$ are always zero except when the learning agent reaches certain crucial states, which are difficult to reach by purely random exploration. 
%
This problem setting, although more practical to real world scenarios, contradicts  the fundamental principle of TD-learning. 
%
First, it is challenging to explore ideal states with non-zero rewards. Since most feedbacks $r(s,a)$ are zero, the policy's early estimation of $Q$-functions can be quite random, which cannot serve as effective guidance to reach meaningful states. 
%
Second, even upon receiving sparse rewards, information conveyed in such delayed feedbacks can be difficult to be back-propagated into $Q$-values of actions that were taken long time ago. 
% 

To illustrate the dilemma faced by regular TD-learning in sparse rewards, we evaluate the performance of a standard TD3 algorithm \cite{fujimoto2018addressing} on the same modified MuJuCo tasks where we evaluate \SAIL and other IL baselines. 
%(\judycom{TBD, experiments are still running} ) 
As shown in Figure \ref{fig:ep1-sail-td3}, without the guidance of demonstrations, a TD3 agent stucks with near-random policies.

 
\begin{figure*}[ht]
    \begin{center}  
       % \vskip -0.2in
        \hskip -0.1in
        \begin{minipage}[b]{.27\textwidth}
            \centerline{\includegraphics[width=\columnwidth]{figs/Walker2d-v2-ep1-dynamic-TD3-test.pdf}} 
            %\caption{Walker2d-v2}\label{ep4-walker}
        \end{minipage} %\hskip -0.3in %\qquad  
        \hskip -0.2in
        \begin{minipage}[b]{.27\textwidth}
            \centerline{\includegraphics[width=\columnwidth]{figs/Swimmer-v2-ep1-dynamic-TD3-test.pdf}}
            %\caption{Swimmer-v2}\label{ep4-swimmer}
        \end{minipage} \hskip -0.2in
        \begin{minipage}[b]{.27\textwidth}
            \centerline{\includegraphics[width=\columnwidth]{figs/Halfcheetah-v2-ep1-dynamic-TD3-test.pdf}}
            %\caption{Swimmer-v2}\label{ep4-swimmer}
        \end{minipage} \hskip -0.2in
        \begin{minipage}[b]{.27\textwidth}
            \centerline{\includegraphics[width=\columnwidth]{figs/Hopper-v2-ep1-dynamic-TD3-test.pdf}} 
        \end{minipage}%\qquad   
        %%%%%%% 
    \caption{Evaluation curves of \SAIL and TD3 with sparse (episodic) rewards, where \SAIL uses one demonstration trajectory.}
    \label{fig:ep1-sail-td3} 
    \end{center}
    \vskip -0.2in
\end{figure*}

\section{Relation to Reward Shaping} 
In addition to Imitation Learning (IL), our approach also draws a connection to Reward Shaping (RS). RS is a widely adopted approach to leverage prior knowledge to facilitate policy learning, especially for tasks with sparse external rewards.
%
RS approach can be formulated as augmenting the environment reward $r$ with an auxiliary term $F$ scaled by coefficient $\lambda> 0 $ \cite{ng1999policy}: 
\begin{align*}
    r'(s,a, s') &= r(s,a) + \lambda F(s,a,s')
\end{align*}
%
In vanilla RS, the auxiliary reward function $F$ takes the form of the difference of the value of \textit{potential function} $\Phi$, with $F(s,a,s') = \gamma \Phi(s') - \Phi(s)$ \cite{ng1999policy}. 
%
The potential function $\Phi$ is an instantiation of prior knowledge to guide the learning policy for efficient exploration. Earlier work focused on \textit{state-dependent} potential function, which can navigate the learning agent to beneficial states.
%
Later work along this line extends the potential to be \textit{action-dependent} \cite{wiewiora2003principled}:  
\begin{align*}
	F(s, a, s', a') = \gamma \Phi(s', a') - \Phi(s, a) 
\end{align*}
%
Action-dependent potential can provide more guidance on whether certain state-actions are beneficial or not.
%
\citet{devlin2012dynamic} extended RS to dynamic potential-based shaping, which allows the shaping function changing over time: 
\begin{align*}
	F(s, t, s', t') = \gamma \Phi(s', t') - \Phi(s, t)
\end{align*}
Considering both action-dependent and time-dependent shaping, a more general form is provided in~\citep{harutyunyan2015expressing} as follows:
\begin{align*}
	F(s, a, t, s', a', t') = \gamma \Phi(s', a', t') - \Phi(s, a, t) 
\end{align*}
%
Although \textit{potential-based} RS has been widely adopted in prior arts \cite{ng1999policy,wiewiora2003principled,devlin2012dynamic}, very limited light has been shed on how to choose a proper potential function $\Phi$. 

The principle of RS has been utilized to different IL and LfD algorithms as well as applications \cite{brys2015reinforcement,kang2018policy,gu2017deep}. From this perspective, \SAIL is also analogous to RS, as they both alter the reward function to encourage efficient exploration in sparse rewarded tasks. 
%
However, \SAIL differs from standard RS approaches in that \SAIL does not necessarily follow the routine of potential-based shaping.  
%
Besides, \SAIL does not hinge on the environment feedback $r$ to build the shaped reward, as in our case, $r'(s,a,.) = -\log(1-D(s,a))$ purely depends on the output from the discriminator $D$. 

Disregarding environment rewards, especially when they are extremely sparse and noisy, serves as a more beneficial strategy than combing them for reward shaping. 
%
Moreover, the scale of environment rewards and shaped rewards may not be comparable, which throws practical challenges to tune a proper coefficient $\lambda$ that is applicable across different tasks. 
%
To illustrate this, consider Figure \ref{fig:ep1-sail-dynamic}, where the on-policy baseline \textit{POfD} (magenta line) combines both environment rewards and discriminator rewards, and GAIL (green line) only adopts discriminator rewards. For \textit{POfD}, we adopt the same scaling coefficient $\lambda$ for different tasks with extremely sparse environment rewards. Compared with GAIL, the performance of \textit{POfD} is unstable. 


==> sections/style.tex <==
\section{Electronic Submission}
\label{submission}

Submission to ICML 2019 will be entirely electronic, via a web site
(not email). Information about the submission process and \LaTeX\ templates
are available on the conference web site at:
\begin{center}
\textbf{\texttt{http://icml.cc/}}
\end{center}

The guidelines below will be enforced for initial submissions and
camera-ready copies. Here is a brief summary:
\begin{itemize}
\item Submissions must be in PDF\@.
\item Submitted papers can be up to eight pages long, not including references, and up to twelve pages when references and acknowledgments are included. Any paper exceeding this length will automatically be rejected. 
\item \textbf{Do not include author information or acknowledgements} in your
    initial submission.
\item Your paper should be in \textbf{10 point Times font}.
\item Make sure your PDF file only uses Type-1 fonts.
\item Place figure captions \emph{under} the figure (and omit titles from inside
    the graphic file itself). Place table captions \emph{over} the table.
\item References must include page numbers whenever possible and be as complete
    as possible. Place multiple citations in chronological order.
\item Do not alter the style template; in particular, do not compress the paper
    format by reducing the vertical spaces.
\item Keep your abstract brief and self-contained, one paragraph and roughly
    4--6 sentences. Gross violations will require correction at the
    camera-ready phase. The title should have content words capitalized.
\end{itemize}

\subsection{Submitting Papers}

\textbf{Paper Deadline:} The deadline for paper submission that is
advertised on the conference website is strict. If your full,
anonymized, submission does not reach us on time, it will not be
considered for publication. 

\textbf{Anonymous Submission:} ICML uses double-blind review: no identifying
author information may appear on the title page or in the paper
itself. Section~\ref{author info} gives further details.

\textbf{Simultaneous Submission:} ICML will not accept any paper which,
at the time of submission, is under review for another conference or
has already been published. This policy also applies to papers that
overlap substantially in technical content with conference papers
under review or previously published. ICML submissions must not be
submitted to other conferences during ICML's review period. Authors
may submit to ICML substantially different versions of journal papers
that are currently under review by the journal, but not yet accepted
at the time of submission. Informal publications, such as technical
reports or papers in workshop proceedings which do not appear in
print, do not fall under these restrictions.

\medskip

Authors must provide their manuscripts in \textbf{PDF} format.
Furthermore, please make sure that files contain only embedded Type-1 fonts
(e.g.,~using the program \texttt{pdffonts} in linux or using
File/DocumentProperties/Fonts in Acrobat). Other fonts (like Type-3)
might come from graphics files imported into the document.

Authors using \textbf{Word} must convert their document to PDF\@. Most
of the latest versions of Word have the facility to do this
automatically. Submissions will not be accepted in Word format or any
format other than PDF\@. Really. We're not joking. Don't send Word.

Those who use \textbf{\LaTeX} should avoid including Type-3 fonts.
Those using \texttt{latex} and \texttt{dvips} may need the following
two commands:

{\footnotesize
\begin{verbatim}
dvips -Ppdf -tletter -G0 -o paper.ps paper.dvi
ps2pdf paper.ps
\end{verbatim}}
It is a zero following the ``-G'', which tells dvips to use
the config.pdf file. Newer \TeX\ distributions don't always need this
option.

Using \texttt{pdflatex} rather than \texttt{latex}, often gives better
results. This program avoids the Type-3 font problem, and supports more
advanced features in the \texttt{microtype} package.

\textbf{Graphics files} should be a reasonable size, and included from
an appropriate format. Use vector formats (.eps/.pdf) for plots,
lossless bitmap formats (.png) for raster graphics with sharp lines, and
jpeg for photo-like images.

The style file uses the \texttt{hyperref} package to make clickable
links in documents. If this causes problems for you, add
\texttt{nohyperref} as one of the options to the \texttt{icml2019}
usepackage statement.


\subsection{Submitting Final Camera-Ready Copy}

The final versions of papers accepted for publication should follow the
same format and naming convention as initial submissions, except that
author information (names and affiliations) should be given. See
Section~\ref{final author} for formatting instructions.

The footnote, ``Preliminary work. Under review by the International
Conference on Machine Learning (ICML). Do not distribute.'' must be
modified to ``\textit{Proceedings of the
$\mathit{36}^{th}$ International Conference on Machine Learning},
Long Beach, USA, 2019.
Copyright 2019 by the author(s).''

For those using the \textbf{\LaTeX} style file, this change (and others) is
handled automatically by simply changing
$\mathtt{\backslash usepackage\{icml2019\}}$ to
$$\mathtt{\backslash usepackage[accepted]\{icml2019\}}$$
Authors using \textbf{Word} must edit the
footnote on the first page of the document themselves.

Camera-ready copies should have the title of the paper as running head
on each page except the first one. The running title consists of a
single line centered above a horizontal rule which is $1$~point thick.
The running head should be centered, bold and in $9$~point type. The
rule should be $10$~points above the main text. For those using the
\textbf{\LaTeX} style file, the original title is automatically set as running
head using the \texttt{fancyhdr} package which is included in the ICML
2019 style file package. In case that the original title exceeds the
size restrictions, a shorter form can be supplied by using

\verb|\icmltitlerunning{...}|

just before $\mathtt{\backslash begin\{document\}}$.
Authors using \textbf{Word} must edit the header of the document themselves.

\section{Format of the Paper}

All submissions must follow the specified format.

\subsection{Length and Dimensions}

Submitted papers can be up to eight pages long, not including references, and up to twelve pages when references and acknowledgments are included.
Acknowledgements should be limited to grants and people who contributed to the paper.
Any submission that exceeds
this page limit, or that diverges significantly from the specified format,
will be rejected without review.

The text of the paper should be formatted in two columns, with an
overall width of 6.75~inches, height of 9.0~inches, and 0.25~inches
between the columns. The left margin should be 0.75~inches and the top
margin 1.0~inch (2.54~cm). The right and bottom margins will depend on
whether you print on US letter or A4 paper, but all final versions
must be produced for US letter size.

The paper body should be set in 10~point type with a vertical spacing
of 11~points. Please use Times typeface throughout the text.

\subsection{Title}

The paper title should be set in 14~point bold type and centered
between two horizontal rules that are 1~point thick, with 1.0~inch
between the top rule and the top edge of the page. Capitalize the
first letter of content words and put the rest of the title in lower
case.

\subsection{Author Information for Submission}
\label{author info}

ICML uses double-blind review, so author information must not appear. If
you are using \LaTeX\/ and the \texttt{icml2019.sty} file, use
\verb+\icmlauthor{...}+ to specify authors and \verb+\icmlaffiliation{...}+ to specify affiliations. (Read the TeX code used to produce this document for an example usage.) The author information
will not be printed unless \texttt{accepted} is passed as an argument to the
style file.
Submissions that include the author information will not
be reviewed.

\subsubsection{Self-Citations}

If you are citing published papers for which you are an author, refer
to yourself in the third person. In particular, do not use phrases
that reveal your identity (e.g., ``in previous work \cite{langley00}, we
have shown \ldots'').

Do not anonymize citations in the reference section. The only exception are manuscripts that are
not yet published (e.g., under submission). If you choose to refer to
such unpublished manuscripts \cite{anonymous}, anonymized copies have
to be submitted
as Supplementary Material via CMT\@. However, keep in mind that an ICML
paper should be self contained and should contain sufficient detail
for the reviewers to evaluate the work. In particular, reviewers are
not required to look at the Supplementary Material when writing their
review.

\subsubsection{Camera-Ready Author Information}
\label{final author}

If a paper is accepted, a final camera-ready copy must be prepared.
%
For camera-ready papers, author information should start 0.3~inches below the
bottom rule surrounding the title. The authors' names should appear in 10~point
bold type, in a row, separated by white space, and centered. Author names should
not be broken across lines. Unbolded superscripted numbers, starting 1, should
be used to refer to affiliations.

Affiliations should be numbered in the order of appearance. A single footnote
block of text should be used to list all the affiliations. (Academic
affiliations should list Department, University, City, State/Region, Country.
Similarly for industrial affiliations.)

Each distinct affiliations should be listed once. If an author has multiple
affiliations, multiple superscripts should be placed after the name, separated
by thin spaces. If the authors would like to highlight equal contribution by
multiple first authors, those authors should have an asterisk placed after their
name in superscript, and the term ``\textsuperscript{*}Equal contribution"
should be placed in the footnote block ahead of the list of affiliations. A
list of corresponding authors and their emails (in the format Full Name
\textless{}email@domain.com\textgreater{}) can follow the list of affiliations.
Ideally only one or two names should be listed.

A sample file with author names is included in the ICML2019 style file
package. Turn on the \texttt{[accepted]} option to the stylefile to
see the names rendered. All of the guidelines above are implemented
by the \LaTeX\ style file.

\subsection{Abstract}

The paper abstract should begin in the left column, 0.4~inches below the final
address. The heading `Abstract' should be centered, bold, and in 11~point type.
The abstract body should use 10~point type, with a vertical spacing of
11~points, and should be indented 0.25~inches more than normal on left-hand and
right-hand margins. Insert 0.4~inches of blank space after the body. Keep your
abstract brief and self-contained, limiting it to one paragraph and roughly 4--6
sentences. Gross violations will require correction at the camera-ready phase.

\subsection{Partitioning the Text}

You should organize your paper into sections and paragraphs to help
readers place a structure on the material and understand its
contributions.

\subsubsection{Sections and Subsections}

Section headings should be numbered, flush left, and set in 11~pt bold
type with the content words capitalized. Leave 0.25~inches of space
before the heading and 0.15~inches after the heading.

Similarly, subsection headings should be numbered, flush left, and set
in 10~pt bold type with the content words capitalized. Leave
0.2~inches of space before the heading and 0.13~inches afterward.

Finally, subsubsection headings should be numbered, flush left, and
set in 10~pt small caps with the content words capitalized. Leave
0.18~inches of space before the heading and 0.1~inches after the
heading.

Please use no more than three levels of headings.

\subsubsection{Paragraphs and Footnotes}

Within each section or subsection, you should further partition the
paper into paragraphs. Do not indent the first line of a given
paragraph, but insert a blank line between succeeding ones.

You can use footnotes\footnote{Footnotes
should be complete sentences.} to provide readers with additional
information about a topic without interrupting the flow of the paper.
Indicate footnotes with a number in the text where the point is most
relevant. Place the footnote in 9~point type at the bottom of the
column in which it appears. Precede the first footnote in a column
with a horizontal rule of 0.8~inches.\footnote{Multiple footnotes can
appear in each column, in the same order as they appear in the text,
but spread them across columns and pages if possible.}

\begin{figure}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{icml_numpapers}}
\caption{Historical locations and number of accepted papers for International
Machine Learning Conferences (ICML 1993 -- ICML 2008) and International
Workshops on Machine Learning (ML 1988 -- ML 1992). At the time this figure was
produced, the number of accepted papers for ICML 2008 was unknown and instead
estimated.}
\label{icml-historical}
\end{center}
\vskip -0.2in
\end{figure}

\subsection{Figures}

You may want to include figures in the paper to illustrate
your approach and results. Such artwork should be centered,
legible, and separated from the text. Lines should be dark and at
least 0.5~points thick for purposes of reproduction, and text should
not appear on a gray background.

Label all distinct components of each figure. If the figure takes the
form of a graph, then give a name for each axis and include a legend
that briefly describes each curve. Do not include a title inside the
figure; instead, the caption should serve this function.

Number figures sequentially, placing the figure number and caption
\emph{after} the graphics, with at least 0.1~inches of space before
the caption and 0.1~inches after it, as in
Figure~\ref{icml-historical}. The figure caption should be set in
9~point type and centered unless it runs two or more lines, in which
case it should be flush left. You may float figures to the top or
bottom of a column, and you may set wide figures across both columns
(use the environment \texttt{figure*} in \LaTeX). Always place
two-column figures at the top or bottom of the page.

\subsection{Algorithms}

If you are using \LaTeX, please use the ``algorithm'' and ``algorithmic''
environments to format pseudocode. These require
the corresponding stylefiles, algorithm.sty and
algorithmic.sty, which are supplied with this package.
Algorithm~\ref{alg:example} shows an example.

\begin{algorithm}[tb]
   \caption{Bubble Sort}
   \label{alg:example}
\begin{algorithmic}
   \STATE {\bfseries Input:} data $x_i$, size $m$
   \REPEAT
   \STATE Initialize $noChange = true$.
   \FOR{$i=1$ {\bfseries to} $m-1$}
   \IF{$x_i > x_{i+1}$}
   \STATE Swap $x_i$ and $x_{i+1}$
   \STATE $noChange = false$
   \ENDIF
   \ENDFOR
   \UNTIL{$noChange$ is $true$}
\end{algorithmic}
\end{algorithm}

\subsection{Tables}

You may also want to include tables that summarize material. Like
figures, these should be centered, legible, and numbered consecutively.
However, place the title \emph{above} the table with at least
0.1~inches of space before the title and the same after it, as in
Table~\ref{sample-table}. The table title should be set in 9~point
type and centered unless it runs two or more lines, in which case it
should be flush left.

% Note use of \abovespace and \belowspace to get reasonable spacing
% above and below tabular lines.

\begin{table}[t]
\caption{Classification accuracies for naive Bayes and flexible
Bayes on various data sets.}
\label{sample-table}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\toprule
Data set & Naive & Flexible & Better? \\
\midrule
Breast    & 95.9$\pm$ 0.2& 96.7$\pm$ 0.2& $\surd$ \\
Cleveland & 83.3$\pm$ 0.6& 80.0$\pm$ 0.6& $\times$\\
Glass2    & 61.9$\pm$ 1.4& 83.8$\pm$ 0.7& $\surd$ \\
Credit    & 74.8$\pm$ 0.5& 78.3$\pm$ 0.6&         \\
Horse     & 73.3$\pm$ 0.9& 69.7$\pm$ 1.0& $\times$\\
Meta      & 67.1$\pm$ 0.6& 76.5$\pm$ 0.5& $\surd$ \\
Pima      & 75.1$\pm$ 0.6& 73.9$\pm$ 0.5&         \\
Vehicle   & 44.9$\pm$ 0.6& 61.5$\pm$ 0.4& $\surd$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

Tables contain textual material, whereas figures contain graphical material.
Specify the contents of each row and column in the table's topmost
row. Again, you may float tables to a column's top or bottom, and set
wide tables across both columns. Place two-column tables at the
top or bottom of the page.

\subsection{Citations and References}

Please use APA reference format regardless of your formatter
or word processor. If you rely on the \LaTeX\/ bibliographic
facility, use \texttt{natbib.sty} and \texttt{icml2019.bst}
included in the style-file package to obtain this format.

Citations within the text should include the authors' last names and
year. If the authors' names are included in the sentence, place only
the year in parentheses, for example when referencing Arthur Samuel's
pioneering work \yrcite{Samuel59}. Otherwise place the entire
reference in parentheses with the authors and year separated by a
comma \cite{Samuel59}. List multiple references separated by
semicolons \cite{kearns89,Samuel59,mitchell80}. Use the `et~al.'
construct only for citations with three or more authors or after
listing all authors to a publication in an earlier reference \cite{MachineLearningI}.

Authors should cite their own work in the third person
in the initial version of their paper submitted for blind review.
Please refer to Section~\ref{author info} for detailed instructions on how to
cite your own papers.

Use an unnumbered first-level section heading for the references, and use a
hanging indent style, with the first line of the reference flush against the
left margin and subsequent lines indented by 10 points. The references at the
end of this document give examples for journal articles \cite{Samuel59},
conference publications \cite{langley00}, book chapters \cite{Newell81}, books
\cite{DudaHart2nd}, edited volumes \cite{MachineLearningI}, technical reports
\cite{mitchell80}, and dissertations \cite{kearns89}.

Alphabetize references by the surnames of the first authors, with
single author entries preceding multiple author entries. Order
references for the same authors by year of publication, with the
earliest first. Make sure that each reference includes all relevant
information (e.g., page numbers).

Please put some effort into making references complete, presentable, and
consistent. If using bibtex, please protect capital letters of names and
abbreviations in titles, for example, use \{B\}ayesian or \{L\}ipschitz
in your .bib file.

\subsection{Software and Data}

We strongly encourage the publication of software and data with the
camera-ready version of the paper whenever appropriate. This can be
done by including a URL in the camera-ready copy. However, do not
include URLs that reveal your institution or identity in your
submission for review. Instead, provide an anonymous URL or upload
the material as ``Supplementary Material'' into the CMT reviewing
system. Note that reviewers are not required to look at this material
when writing their review.
